Error Discovery by Clustering Influence Embeddings

We present a method for identifying groups of test examples -- slices -- on which a model under-performs, a task now known as slice discovery. We formalize coherence -- a requirement that erroneous predictions, within a slice, should be wrong for the same reason -- as a key property that any slice discovery method should satisfy. We then use influence functions to derive a new slice discovery method, InfEmbed, which satisfies coherence by returning slices whose examples are influenced similarly by the training data. InfEmbed is simple, and consists of applying K-Means clustering to a novel representation we deem influence embeddings. We show InfEmbed outperforms current state-of-the-art methods on 2 benchmarks, and is effective for model debugging across several case studies.

==> sections/covid.tex <==
\paragraph{Diagnosing Multiple Errors: Mislabelled Examples \& Spurious Correlation} We extend the experiments above to a setting where there are multiple types of errors with the training data and model. Specifically, in addition to a spurious signal, we also corrupt a specific class via training set mislabeling. Consequently the model underperforms on two groups of data for different reasons. We consider the background blur as a spurious signal for the Mid/Early Puberty class, and mislabelling for the toddler class. We refer to Section~\ref{appendix:rad:results} for additional details.

\textbf{Results.} We find that we are able to recover $3$ underperforming slices. Two slices correspond to mislabelled examples, and the last captures errors due to background blur.

\subsection{Applying Influence Embeddings to Limited Data Settings and Using Attributes} 
We now a previously unconsidered setting; one where the test dataset used to perform slice discovery is small, and we have additional attributes/annotations for that small dataset. Here, we show \texttt{InfEmbed} is still able to distinguish high-performing vs. low ones, and that annotations help provide metadata for characterizing the clusters observed.

%\begin{figure}[t]
%\centering
%\includegraphics[page=2, scale=0.45]%{figures/influence_embedding_compressed.pdf}
%\label{fig:imagenet}
%\caption{\textbf{Two false positives samples identified in each of the three clusters. Each row denotes a different cluster.}}
%\label{fig:fp}
%\end{figure}

\textbf{Overview \& Experimental Procedure}: We consider the test split of the COVID-19 Chest X-Ray Dataset\footnote{ https://github.com/ieee8023/covid-chestxray-dataset}, which only has 107 examples.  The pre-trained model we analyze is a resnet50 model, obtained by fine tuning a model trained to predict multiple diseases to the COVID-19 task via fine tuning.  All models and data come from the torchxrayvision library. The model achieves an accuracy of 76.6\% on the test set of 107 points. We apply \texttt{InfEmbed} with $K=3$, and Arnoldi dimension $P=250$, influence embedding dimension $D=125$.

\textbf{Results}:
The first cluster had an accuracy of 85\%, capturing the majority of correctly classified samples. The second cluster consisted of four samples that were false positives and two samples that were true negatives, while the third cluster had six samples that were false positives, and one sample that was a false negative. Using additional metadata regarding additional diseases and infections(See Table \ref{tab:covid_labels} in Appendix), we find that the key differentiator between the three clusters is the incidence of additional diseases. Some false positive samples in cluster 2, in addition to pneumonia and tuberculosis, also had legionella, while those in cluster 3 in addition had SARS or pneumocystis. Taken together, we find that additional metadata can help point out cluster differences that go beyond performance values.

==> sections/old/background_icml.tex <==
\section{Background\label{sec:background}}
Here, we describe the slice discovery problem, influence functions, and how to approximate the inverse Hessian using the Arnoldi iteration---a key component of our method.

%\textbf{Slice Discovery Problem:} In the slice discovery problem, one is given a pre-trained \emph{multi-class} classification model $f(\boldsymbol{\cdot};\theta)$, where $\theta$ denotes the model's real-valued parameters.  Given an example $x\in\mathcal{X}$, some input space (i.e. image, text), $f(x;\theta)\in \mathbb{R}^C$ is the prediction for the example, where $C$ is the number of possible classes, and $f(x;\theta)_c$ is the pre-softmax prediction for class $c$.  One is also given a test dataset with $N$ examples $\te{\mybold{Z}}\coloneqq[\idx{\te{z}}{1},\mydots,\idx{\te{z}}{N}]$, where $\idx{\te{z}}{i}\coloneqq (\idx{\te{x}}{i},\idx{\te{y}}{i})$ with $\idx{\te{x}}{i}\in\mathcal{X}$, $\idx{\te{y}}{i}\in [0,1]^{C}$, on which the model makes predictions $\idx{\hat{\te{y}}}{i} \coloneqq \operatorname{argmax}_c f(\idx{\te{x}}{i})_c$.  Given the model $f(\boldsymbol{\cdot};\theta)$ and test dataset $\mybold{\te{Z}}$, the goal of the slice discovery problem is to produce a partition of the test dataset into $K$ slices: $\{\Phi_k\}_{k=1}^K$, where $\Phi_k \subseteq [N]$, $\Phi_k \cap \Phi_{k'}=\emptyset$ for $k\neq k'$, $\cup_{k=1}^K \Phi_k = [N].$  As we will make precise shortly, each slice $\Phi_k$ should be coherent, and some slices should be under-performing slices in that the error rate $\tfrac{1}{|\Phi_k|}\sum_{i\in\Phi_k}1[\idx{\te{y}}{i} \neq \idx{\hat{\te{y}}}{i}]$ should be high.  Finally, the model is assumed to be trained on a training dataset with $\tr{N}$ examples, $\tr{\mybold{Z}}\coloneqq[\idx{\tr{z}}{1},\mydots,\idx{\tr{z}}{\tr{N}}]$ using cross-entropy loss, so that $\theta = \operatorname{argmin}_{\theta'}\tfrac{1}{\tr{N}}\sum_{i=1}^{\tr{N}}L(\idx{\tr{z}}{i}; \theta')$.  Here, $\idx{\tr{z}}{i}\coloneqq (\idx{\tr{x}}{i},\idx{\tr{y}}{i})$ with $\idx{\tr{x}}{i}\in\mathcal{X}, \idx{\tr{y}}{i}\in[C]$, and given $z\coloneqq(x,y)$, $L(z;\theta)\coloneqq \log \textstyle \sum_c (y)_c \tfrac{\exp(f(x;\theta)_c)}{\sum_c \exp(f(x;\theta)_c)}$.  Note that our definition of the problem assumes training data is available, as it is used to define what it means for a slice to be coherent.

\textbf{Slice Discovery Problem:} In the slice discovery problem, we have a pre-trained \emph{multi-class} classification model $f(\boldsymbol{\cdot};\theta)$, where $\theta$ is the model's real-valued parameters.  Given example $x\in\mathcal{X}$, some input space, $f(x;\theta)\in \mathbb{R}^C$ is the prediction for the example, where $C$ is the number of classes, and $f(x;\theta)_c$ is the pre-softmax prediction for class $c$.  We are also given a test dataset with $N$ examples $\te{\mybold{Z}}\coloneqq[\idx{\te{z}}{1},\mydots,\idx{\te{z}}{N}]$, where $\idx{\te{z}}{i}\coloneqq (\idx{\te{x}}{i},\idx{\te{y}}{i})$ with $\idx{\te{x}}{i}\in\mathcal{X}$, $\idx{\te{y}}{i}\in \mathcal{Y}\coloneqq[0,1]^{C}$.  Given the model $f(\boldsymbol{\cdot};\theta)$ and test dataset $\mybold{\te{Z}}$, the goal of the slice discovery problem is to partition the test dataset into $K$ slices: $\{\Phi_k\}_{k=1}^K$, where $\Phi_k \subseteq [N]$, $\Phi_k \cap \Phi_{k'}=\emptyset$ for $k\neq k'$, $\cup_{k=1}^K \Phi_k = [N].$  As we will make precise shortly, each slice $\Phi_k$ should be coherent, and some slices should be under-performing slices. The model is assumed to be trained on a training dataset with $\tr{N}$ examples, $\tr{\mybold{Z}}\coloneqq[\idx{\tr{z}}{1},\mydots,\idx{\tr{z}}{\tr{N}}]$ where $\idx{\tr{z}}{i}\coloneqq (\idx{\tr{x}}{i},\idx{\tr{y}}{i})$ with $\idx{\tr{x}}{i}\in\mathcal{X}, \idx{\tr{y}}{i}\in\mathcal{Y}$, so that $\theta = \operatorname{argmin}_{\theta'}\tfrac{1}{\tr{N}}\sum_{i\shorteq1}^{\tr{N}}L(\idx{\tr{z}}{i}; \theta')$. We assume loss function $L$ is cross-entropy loss.  Thus, given $z=(x,y)$ with $x\in\mathcal{X}, y=[y_1,\mydots,y_C]\in \mathcal{Y}$, $L(z;\theta) = -\textstyle \sum_c y_c \log p_c$, with $p=[p_1,\mydots,p_C]$ and $p_c\coloneqq \tfrac{\exp(f(x;\theta)_c)}{\sum_{c'} \exp(f(x;\theta)_{c'}))}$, i.e. $p=\operatorname{softmax}(f(x;\theta))$.

\textbf{Influence Functions}: Formally, given a training example $\tr{z}$ and test example $\te{z}$, one seeks $L(\te{z};\theta)\shortsub L(\te{z};\theta_{\backslash \tr{z}})$, 
where 

$\theta_{\backslash \tr{z}}\coloneqq \operatorname{argmin}_{\theta'}\sum_{i=1}^{\tr{N}} 1[\idx{\tr{z}}{i} \shortneq \tr{z}]L(\idx{\tr{z}}{i};\theta')$ 
is the model parameter obtained from retraining with $\tr{z}$ removed. 
Influence functions approximate this quantity via first-order approximation: the effect of infinitesimal down-weighting of $\tr{z}$ followed by retraining. Define $\theta_{\tr{z},\epsilon}\coloneqq \operatorname{argmin}_{\theta'}\sum_{i=1}^{\tr{N}} L(\idx{\tr{z}}{i};\theta') + \epsilon L(\tr{z};\theta')$. 

\citet{koh2017understanding} show the Jacobian $\tfrac{d\theta_{\tr{z},\epsilon}}{d\epsilon} = \nabla_{\theta} L(\tr{z};\theta)^{\intercal} H_{\theta}^{-1}$, where $H_{\theta}\coloneqq \sum_{i=1}^{\tr{N}} \nabla_{\theta}^2 L(\idx{\tr{z}}{i};\theta)$ is the Hessian.  Applying the chain rule gives the influence of training example $\tr{z}$ on test example $\te{z}$:
\begin{align}
I(\tr{z},\te{z}) \coloneqq \nabla_{\theta} L(\tr{z};\theta)^{\intercal} H_{\theta}^{-1} \nabla_{\theta} L(\te{z};\theta).\label{eq:influence}
\end{align}

\textbf{Practical Low-Rank Influence Function:} The main challenge in computing influence is that it is impractical to explicitly form the $H_{\theta}$ needed to compute influence in Equation \ref{eq:influence} unless the model is small, or if one only considers parameters in a few layers. \citet{schioppa2022scaling} address this problem by forming a low-rank approximation of $H_{\theta}^{-1}$ via a procedure that does not explicitly form $H_{\theta}$. In brief, they run the Arnoldi iteration \cite{trefethen1997numerical} for $P$ iterations to get a $P$-dimensional Krylov subspace for $H_{\theta}$, which requires only $P$ Hessian-vector products.  Then, they find a rank-$D$ approximation of the restriction of $H_{\theta}$ to the Krylov subspace, a small $P\times P$ matrix, via eigendecomposition.  Their procedure is summarized by an algorithm $\operatorname{FactorHessian}$ (Appendix Section \ref{appendix:lowinf} has details), which returns factors of a low-rank approximation of $H_{\theta}^{-1}$
\begin{align}
M, \lambda &= \operatorname{FactorHessian}(\tr{\mybold{Z}}, \Theta, P, D)\ \text{where}\label{eq:factors}\\
\hat{H}_{\theta}^{-1} &\coloneqq M\lambda^{-1}M^{\intercal} \approx H_{\theta}^{-1}, \label{eq:H_hat}
\end{align}
$M \in \mathbb{R}^{|\theta|\times D}$, $\lambda \in \mathbb{R}^{D\times D}$ is an easily-invertible \emph{diagonal} matrix, $|\theta|$ is the number of parameters, $\hat{H}_{\theta}^{-1}$ approximates $H_{\theta}^{-1}$, $D$ is the rank of the approximation, $P$ is the Arnoldi dimension, i.e. number of Arnoldi iterations, and here and everywhere, \emph{configuration} $\Theta\coloneqq(L,f,\theta)$ denotes the loss function, model, parameters.  $\hat{H}_{\theta}^{-1}$ is then used to define the \emph{practical influence} of training example $\tr{z}$ on test \mbox{example $\te{z}$:}
\begin{align}
\hat{I}(\tr{z},\te{z}) &\coloneqq \nabla_{\theta} L(\tr{z};\theta)^{\intercal} \hat{H}_{\theta}^{-1} \nabla_{\theta} L(\te{z};\theta).\label{eq:influence_hat}
\end{align}

%Their low-rank implementation first applied the Arnoldi iteration \cite{trefethen1997numerical} to compute an orthonormal basis $(q_1,\mydots,q_D)$ for the $P$-dimensional Arnoldi subspace $(b,H_{\theta}b,\mydots,H_{\theta}^{P-1})$, as well as the restriction $R$ of $H_\theta$ to the subspace, so that $H_{\theta}=QRQ^{\intercal}$, where $Q\coloneqq [q_1,\mydots,q_P] \in \mathbb{R}^{|\theta|\times P}$ and $R \in \mathbb{R}^{P\times P}$. They then approximate %$R\approx V\lambda V^{\intercal}$ and
%$R^{-1}\approx V\lambda^{-1} V^{\intercal}$, where $V=[v_1,\mydots,v_D]\in\mathbb{R}^{P \times D}$, $v_1,\mydots,v_D$ are the top $D$ eigenvectors of $R$, and $\lambda=\operatorname{diag}(\lambda_1,\mydots,\lambda_D)$, where $\lambda_1,\mydots,\lambda_D$ are the corresponding eigenvalues. Finally, they form a low-rank approximation of $H_{\theta}^{-1}$, 
%\begin{align}
%\hat{H}_{\theta}^{-1} &\coloneqq M\lambda^{-1}M^{\intercal},\ \text{where}\ M=QV\label{eq:H_hat}
%\intertext{and use it to define the \emph{practical influence} of training example $\tr{z}$ on test example $\te{z}$:}
%\hat{I}(\tr{z},\te{z}) &\coloneqq \nabla_{\theta} L(\tr{z};\theta)^{\intercal} \hat{H}_{\theta}^{-1} \nabla_{\theta} L(\te{z};\theta).\label{eq:influence_hat}
%\end{align}
%To compute practical influence, one thus pre-computes the factors of $\hat{H}_{\theta}^{-1}$.  Pseudocode for this computation, a function $\operatorname{FactorHessian}(\tr{\mybold{Z}}, \Theta, P, D)$ returning the factors $M,V$ of Equation \ref{eq:H_hat} is in Algorithm \ref{alg:arnoldi_factor} of the Appendix, where $P$ is the Arnoldi dimension, $D$ is the dimension of the low-rank approximation.  Here and elsewhere, we let $\Theta\coloneqq(L,f,\theta)$ denote the loss function, model, and parameters.

%Algorithm \ref{alg:arnoldi_factor} outlines finding the factors needed for $\hat{H}_{\theta}^{-1}$.  For brevity, throughout we will let \emph{configuration} $\Theta\coloneqq(L,f,\theta)$ denote the loss %function, model, and parameters.
%computing it once, caching its factors $QV$ and $\lambda^{-1}$, and substituting the approximation in Equation \ref{eq:influence}:
%\begin{align}H_{\theta}^{-1} \approx QV\lambda^{-1}V^{\intercal}Q^{\intercal}.
%\end{align}
%Because it is impractical to even form the requisite $H_{\theta}$, existing influence function implementations only require access to Hessian-vector products when computing influence, i.e. compute $H_{\theta}v$ for an arbitrary v.


==> sections/old/experiments_icml.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Baselines
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Comparing \texttt{InfEmbed} to Baselines}
In this section, we present quantitative comparisons of \texttt{Inf-Embed} method of Algorithm~\ref{alg:basic} to several others on two benchmark settings. First, we compare \texttt{Inf-Embed} to Domino~\citep{eyuboglu2022domino} on the \texttt{dcbench} benchmark~\cite{eyuboglu2022dcbench}. Second, we compare to several additional methods on the \texttt{SpotCheck} benchmark~\cite{plumb2022evaluating}. On \texttt{dcbench}, we find that \texttt{Inf-Embed} outperforms Domino across all the three data modalities and all three types of error. On the \texttt{SpotCheck} benchmark, we find that \texttt{Inf-Embed} matches the performance of the current best performing approach.
%%%%%%%%%%%%%%%%%%%%%%%%%%
% Domino Dcbench results
%%%%%%%%%%%%%%%%%%%%%%%%
\begin{wraptable}{r}{9cm}
\centering
\rowcolors{2}{}{lightgray}
\resizebox{.9\linewidth}{!}{
\begin{tabular}{cccc}
\hline
 & \textbf{Rare} & \textbf{Correlation} & \textbf{Noisy Label}\\
\textbf{SDM Approach}   &  &  & \\
\hline
\multicolumn{4}{c}{\textbf{Natural Images}} \\
\hline
\hline
 Domino   & 0.4 &  0.45  & 0.6 \\
Inf-Embed &  0.65 &  0.55 & 0.67   \\
\hline
\multicolumn{4}{c}{\textbf{Medical Images}} \\
\hline
Domino    &  0.39  & 0.6 & 0.58\\
Inf-Embed & 0.57 &  0.62 & 0.73   \\
\hline
\multicolumn{4}{c}{\textbf{Medical Time Series}} \\
\hline
Domino    & 0.6   & 0.55 & 0.9\\
Inf-Embed &  0.64 & 0.65  & 0.81   \\
\hline
\end{tabular}
}
\caption{Comparison between Domino and Influence Embedding Methods on the  \texttt{dcbench} benchmark for trained models across three categories of inputs.}
\label{tab:dominotrainedmodel}
\end{wraptable}

\subsection{\texttt{InfEmbed} on \texttt{dcbench}}
\label{dcbench}

\textbf{Overview \& Experimental Procedure.} \texttt{dcbench}~\citep{eyuboglu2022dcbench} provides 1235 pre-trained models that are derived from data manipulated to exhibit one of three kinds of errors. Since the error causing slice is known, a priori, \texttt{dcbench} can serve as a way to assess a new SDM. The underlying datasets for these tasks include natural images (ImageNet~\cite{deng2009imagenet}, and CelebA~\citep{liu2015deep}), Medical images (MIMIC Chest X-Ray~\citep{johnson2016mimic, johnson2020mimic}), and Medical Time-Series Data (EEG signals~\citep{saab2020weak}).~\citet{eyuboglu2022dcbench} also introduced Domino, the current state-of-the-art on \texttt{dcbench}, an approach that uses multi-model embeddings as input to an error-aware mixture model for partitioning a test data. Following~\citet{eyuboglu2022dcbench}, we compare \texttt{InfEmbed} to Domino using the precision-at-k measure, which measures the proportion of the top k ($k=10$) elements in the discovered slice that are in the ground truth slice. Appendix Section~\ref{appendix:dc} contains additional setup details.

\textbf{Results.} We present the results of comparison to Domino in Table~\ref{tab:dominotrainedmodel}. \texttt{Inf-Embed} beats Domino across all settings except on the Noisy Label task for the EEG data modality. 

\subsection{\texttt{InfEmbed} on the SpotCheck Benchmark}
\label{spotcheck}

%%%%%%%%%%%%%%%%%%%%%%%%%%
% Spotcheck results
%%%%%%%%%%%%%%%%%%%%%%%%
\begin{wraptable}{r}{7.5cm}
\centering
\rowcolors{1}{}{lightgray}
\resizebox{.7\linewidth}{!}{
\begin{tabular}{ccc}
\hline
%\multicolumn{2}{c}{Item} \\
%\cline{1-2}
 & \textbf{DR} & \textbf{FDR} \\
\textbf{SDM Approach}   &  & \\
\hline
Barlow   & 0.43(0.04) &  0.03(0.01) \\
Spotlight &  0.79(0.03) &  0.09 (0.55)  \\
Domino    &  0.64 (0.04)  & 0.07(0.01)\\ 
PlaneSpot & 0.85 (0.03) & 0.07 (0.01) \\
Inf-Embed & 0.91 (0.09) &  0.15 (0.62) \\
\hline
\end{tabular}
}
\caption{Spotcheck Benchmark results.}
\label{tab:spotcheck}
\end{wraptable}

\textbf{Overview \& Experimental Procedure.} The SpotCheck benchmark~\cite{plumb2022evaluating} is based on a synthetic task consisting of 3 semantic features that can be easily controlled to determine the number of `blindspots' in a dataset. A blindspot is feature responsible for a model's mistake. Similar to  \texttt{dcbench}, a model trained on data generated from SpotCheck is induced to make mistakes on an input that has a set of blindspots. The overall task is to predict the presence of a square in the image. Attributes of the input image such as the background, object color, and co-occurrence can be varied to induce mistakes. ~\citet{plumb2022evaluating} find that current SDM approaches struggle in the presence of several blindspots. Consequently, they propose PlaneSpot, an SDM that uses the representation of the model's last layer, projected to 2 dimensions, along with the model's `confidence' as part of a mixture model to partition the dataset. They show that PlaneSpot outperforms current approaches as measured by discovery and false discovery rates. We replicate the SpotCheck benchmark and compare $\operatorname{InfEmbed}$ to PlaneSpot. We refer to the Section~\ref{appendix:sc:datasets} for additional details.


\textbf{Results.} We report the performance of the influence embedding approach compared to PlaneSpot on the Spotcheck benchmark in Table~\ref{tab:spotcheck}. We find that Inf-Embed approaches matches PlaneSpot's performance on the benchmark.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Case Studies
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Applications of \texttt{InfEmbed}}
In this section, we demonstrate the capability of the influence embedding approach across several datasets and scenarios. First, we show that we can scale the approach to realistic datasets and models like ImageNet. Second, we demonstrate that the influence embedding approach can be used to isolate slices whose errors is due to spurious training signals. Crucially, we find that influence embeddings can help identify slices whose error is due to background blur---a setting that proves challenging for current post-hoc explanation approaches. Finally, we show that the addition of meta data can help `explain' clusters.

\begin{figure*}[ht]
\centering
\includegraphics[page=1, scale=0.23]{figures/influence_embedding_compressed.pdf}
\label{fig:imagenet}
\caption{\textbf{Overview of Influence embedding Clustering for a Resnet-18 on ImageNet.} We show two slices from applying the influence embedding approach to the ImageNet data. We apply the $\operatorname{RuleFind}$ algorithm and identify slices with accuracy under $40$ percent and atleast 25 samples. \textbf{Left}: On the left, we show the distribution of labels and model predictions in that slice (Labels are in red, and Prediction are blue). \textbf{Middle}: Representative examples from the slice. \textbf{Right}: We show four opponent examples for the identified slice.}
\end{figure*}

\subsection{Imagenet}
\input{sections/imagenet.tex}

%%%%%%%%%%%
%AGnews
%%%%%%%%%%%
\input{sections/agnews}

\subsection{Detecting Spurious Signals \& Multiple Blindspots}
\textbf{Overview \& Experimental Procedure.} We now turn to the task detecting a model's reliance on spurious training signals. Here, we focus on a set of signals that have been previously discussed in the literature as challenging (See: ~\citet{zhou2022feature} and ~\citet{adebayo2021post}). We consider 5-class boneage classification task\footnote{\url{https://www.kaggle.com/datasets/kmader/rsna-bone-age}} where we inject 3 possible kinds of spurious signals (see Figure~\ref{fig:radspurious}) in the training data, and verify that the corresponding models learn 



We create manipulated versions of the training set where we inject 3 possible kinds of spurious signals (see Figure~\ref{fig:radspurious}), and train models to associate a particular class with each training signal. We consider a boneage 5-class classification task \footnote{\url{https://www.kaggle.com/datasets/kmader/rsna-bone-age}}. At test time, we break the association between the spurious signal and the original training class by testing the model on a dataset that does not have training-time signal.

\textbf{Experimental Procedure.} Similar to the workflow presented in the ImageNet setting, we first apply the \texttt{RuleFind} method of Algorithm \ref{alg:rulefind} and identify slices with accuracy under $40$ percent and that have at least 25 samples. To assess whether RuleFind is successful at alerting that a model is relying on spurious signal we perform two steps: 1) Inspect whether any of the problematic slices returned contain samples that belong to the class for which the model learned to associate the spurious training signal, and 2) to confirm that the wrong predictions in the slice identified are due to spurious signals injected, we inspect the opponents of the problematic slice. If the opponents are mostly training inputs that also contain the spurious signal, it suggests the cause of the errors in the problematic slice is spurious correlation signals in the opponents.

\begin{figure}[t]
\centering
\includegraphics[page=3, scale=0.27]{figures/influence_embedding_compressed.pdf}
\label{fig:imagenet}
\caption{\textbf{Spurious training signals added to the boneage age prediction task.} We show representative images, for the Mid/Early Pre-Puberty Class, of the three spurious signals we consider on the bone-age prediction task.}
\label{fig:radspurious}
\end{figure}

\paragraph{Detecting a Single Spurious Correlation:} We first assess the ability of \texttt{InfEmbed} for error discovery under the setting where a single spurious correlation is responsible for a trained model's mistake. We train a Resnet-50 model on the bone-age dataset, and inject a single spurious signal in the training set to ensure that the model aligns the Early/Mid Pre-Puberty examples with the injected spurious signal. We experimentally confirm that an image with only the spurious signal is predicted as belong to the class Early/Mid Pre-Puberty. We repeat this procedure for three different spurious signals independently: Image Tag, Stripe, and Background Blur, shown in Figure \ref{fig:radspurious}.

\textbf{Results.} In Figure~\ref{fig:raddistproponents}, we show the results of applying the \texttt{RuleFind} method to each spurious model. Specifically, we find that each run of the algorithm returns only 2 clusters as satisfying the pre-defined rule. Across all the settings considered, the worst performing slice contains samples that are pre-dominantly labeled as the class for which spurious signal was aligned. In Figure~\ref{fig:raddistproponents}-left, we show the distribution of model predictions and labels for the most problematic cluster. As expected, we do find that the Early/Mid Puberty dominates the cluster. This is because the Early/Mid Puberty samples in the test set do not include the spurious signal, so the model errs on these samples.

Having established that the \texttt{RuleFind} method can identify the worst performing slice, we seek to establish that the opponents of these slices can help demonstrate that the model is indeed relying on spurious signals.
In Figure~\ref{fig:raddistproponents}-Right, we show the distribution of samples per-class in the top-$50$ opponents of the slice. If the cause of these errors was indeed the spurious signal injected in the training set, then a large fraction of the opponents should correspond to the samples from the class to which the spurious training signal was injected. As expected, across all settings, we find that about $80$ percent of opponents are Early/Mid Pre-Puberty samples. Consequently, slice opponents can be used to diagnose a model's dependence on spurious signals.

\begin{figure}[t]
\centering
\includegraphics[page=4, scale=0.28]{figures/influence_embedding_compressed.pdf}
\label{fig:imagenet}
\caption{\textbf{Model Prediction and Opponent Breakdown for each Spurious signal.}}
\label{fig:raddistproponents}
\end{figure}

==> sections/old/influenceembed_icml.tex <==
\section{Discovering Problematic Slices By Clustering Influence Embeddings}
\label{sec:influenceembeddings}

\subsection{Problem Formulation}
We would like to partition the test data into slices such that predictions for examples in the same slice have similar root causes as quantified by influence functions.  %What should be the formal representation of the root cause of an example's prediction? Leveraging influence functions, the root cause of a test example's prediction due to a given training example is the influence of the given training example on the test example.  
Therefore, we propose to represent the root cause of the prediction for a test example $\te{z}$ with its \emph{influence explanation $E(\te{z})$:}
\begin{align}
E(\te{z}) \coloneqq \{\hat{I}(\idx{\tr{z}}{j},z)\}_{j=1}^{\tr{N}},
\end{align} 
which is the vector containing the practical influence of every training example on the test example.  Thus, test examples with similar influence explanations are ``influenced similarly by the training data".  We then want each slice be \emph{coherent} in the following sense: the Euclidean distance between influence explanations of examples in the same slice tends to be low.

Therefore, we solve the slice discovery problem described in Section \ref{sec:background} via the following formulation---return a partition of the test dataset into slices, $\{\Phi_k\}_{k=1}^K$, that minimizes the total Euclidean distance between influence explanations of examples in the same slice. Formally, we seek:
\begin{align}
\hspace{-4pt}\operatorname{argmin}_{\{\Phi_k\}_{k=1}^K} \textstyle\sum_k \textstyle\sum_{i,i'\in \Phi_k} ||E(\idx{\te{z}}{i}) - E(\idx{\te{z}}{i'})||^2.\label{eq:formulation}
\end{align}

\subsection{Influence Explanations \& Influence Embeddings}
\label{sec:influence_embedding}
To form coherent slices, a naive approach would be to form the influence explanation of each test example, and apply K-Means clustering with Euclidean distance to them.  However, influence explanations are high-dimensional, with dimensionality equal to the size of the training data, $\tr{N}$.  Instead, we will leverage \emph{influence embeddings}: vectors such that the practical influence of a training example on a test example is the dot-product of their respective influence embeddings.  Looking at Equations \ref{eq:H_hat} and \ref{eq:influence_hat}, we see the influence embedding $\mu(z)$ of an example $z$ must be defined as
\begin{align}
\mu(z) \coloneqq \lambda^{-1/2} M^{\intercal}  \nabla_{\theta} L(z;\theta) \label{eq:emb}%\lambda^{1/2}M^{\intercal}\label{eq:emb}
\end{align}
and $M$, $\lambda$ are as defined in Section \ref{sec:background}, because for any training example $\tr{z}$ and test example $\te{z}$, $\hat{I}(\tr{z},\te{z})=\mu(\tr{z})^{\intercal}\mu(\te{z})$.  Procedure \texttt{GetEmbeddings} of Algorithm \ref{alg:basic} finds $D$-dimensional influence embeddings for the test dataset $\te{\mybold{Z}}$, which has runtime \emph{linear} in the Arnoldi dimension $P$.  The rank $D$ of the factors from $\texttt{FactorHessian}$ determines the dimension of the influence embeddings.

%To form coherent slices, we will instead apply K-Means clustering to the influence embeddings of test examples.  This is justified by the following Lemma:

Influence embeddings satisfy a critical property - that if two examples have similar influence embeddings, they also tend to have similar influence explanations.  This is formalized by the following lemma, whose proof follows from the Cauchy-Schwartz inequality, and that influence is the dot-product of influence embeddings (see Appendix Section \ref{appendix:propoppo}) 
\begin{lemma}\label{lemma:emb}
There is a constant $C > 0$ such that for any test examples $\idx{\te{z}}{i},\idx{\te{z}}{j}$, $||E(\idx{\te{z}}{i}) - E(\idx{\te{z}}{j})||^2 \leq C||\mu(\idx{\te{z}}{i}) - \mu(\idx{\te{z}}{j}))||^2$.
\end{lemma}

\subsection{\mbox{Discovering Problematic Slices with \texttt{InfEmbed}}}
We will solve the formulation of Equation \ref{eq:formulation} via a simple procedure which applies K-Means with Euclidean distance to the influence \emph{embeddings} of the test dataset, $\boldsymbol{\mu}\coloneqq[\mu(\te{z}_1),\mydots,\mu(\te{z}_{\te{N}})]$.  This procedure is justified as follows: Using Lemma \ref{lemma:emb}, given any partition $\{\Phi_k\}$, we know
\begin{align}
\textstyle\sum_k \textstyle\sum_{i,i'\in \Phi_k} ||&E(\idx{\te{z}}{i}) - E(\idx{\te{z}}{i'})||^2 \leq\label{eq:lhs} \\C &\textstyle\sum_k \textstyle\sum_{i,i'\in \Phi_k} ||\mu(\idx{\te{z}}{i}) - \mu(\idx{\te{z}}{i'})||^2\label{eq:rhs}.
\end{align}
However, the quantity in Equation \ref{eq:rhs} is the \emph{surrogate} objective minimized by this procedure - it is the K-Means objective applied to influence embeddings, scaled by $C>0$ which does not matter.  The quantity in Equation \ref{eq:lhs} is the \emph{actual} objective which the formulation of Equation \ref{eq:formulation} minimizes.  Therefore, the procedure is minimizing a surrogate objective which upper bounds the actual objective we care about.  Put another way, by applying K-Means to influence embeddings, examples within the same slice will not only have similar influence embeddings, but also similar influence explanations as originally desired, by Lemma \ref{lemma:emb}.
%says that examples with similar influence embeddings also tend to have similar influence explanations.
Algorithm \ref{alg:basic} is the proposed $\operatorname{InfEmbed}$ method.
\begin{algorithm}

\begin{algorithmic}[1]
\caption{Algorithm for Discovering Problematic Slices}
\label{alg:basic}
\Procedure{GetEmbeddings}{$\te{\mybold{Z}},\tr{\mybold{Z}},\Theta,P, D$}
%\State\textbf{Inputs:} training data $\{z'_i\}$, loss function $L$, model $f$, model parameter $\theta$, Arnoldi dimension $P$, rank $D$
\State \textbf{Outputs}: \mbox{$D$-dimensional embeddings for test data $\te{\mybold{Z}}$}
\State $M,\lambda \gets \operatorname{FactorHessian}(\tr{\mybold{Z}}, \Theta, P, D)$
\State $\mu_i \gets \lambda^{-1/2} M^{\intercal} \nabla_\theta L(z_i;\theta)$ for $i=1,\mydots,N$
\State $\boldsymbol{\mu} \gets [\mu_1,\mydots,\mu_N]$
\State \textbf{Return:} $\boldsymbol{\mu}$
\EndProcedure
\Procedure{K-Means}{$\boldsymbol{\mu}, K$}
\State randomly initialize cluster centers $c_1,\mydots,c_K$
\While{not converged}
\State $r_i=\operatorname{argmin}_k ||\mu_i - c_k||^2$ for $\mu_i \in \boldsymbol{\mu}$
\State $c_k=\tfrac{ \sum_i 1[r_i=k] \mu_i}{ \sum_i 1[r_i=k]}$ for $k\in[K]$
\EndWhile
\State \textbf{Return:} $[r_1,\mydots,r_{\te{N}}]$
\EndProcedure

\Procedure{InfEmbed}{K, $\te{\mybold{Z}},\tr{\mybold{Z}},\Theta,P, D$}
%\State\textbf{Inputs:} training data $\{z'_i\}$, loss function $L$, model $f$, model parameter $\theta$, Arnoldi dimension $P$, rank $D$
\State \textbf{Inputs}: number of slices $K$, training dataset $\tr{\mybold{Z}}$, test dataset $\te{\mybold{Z}}$, configuration $\Theta$, Arnoldi dimension $P$, influence embedding dimension $D$
\State \textbf{Outputs}: partition of test dataset into slices, $\Phi$
\State $\boldsymbol{\mu}\gets \operatorname{GetEmbeddings}(\te{\mybold{Z}},\tr{\mybold{Z}},\Theta,P, D)$
\State $[r_1,\mydots,r_{\te{N}}] \gets  \operatorname{K-Means}(\boldsymbol{\mu}, K)$
\State \textbf{Return:} $\{\{i \in [N]: r_i=k\}\ \text{for}\ k\in[K]\}$
\EndProcedure
\caption{Our SDM, \texttt{InfEmbed}, consists of K-Means clustering applied to influence embeddings of test examples.}
\end{algorithmic}
\end{algorithm}

\subsection{\mbox{\texttt{InfEmbed-Rule} - Finding Slices Satisfying a Rule}}
The key hyperparameter of the $\operatorname{InfEmbed}$ method is $K$, the number of slices to return.  In practice, it may not be intuitive for a user to choose $K$.  Instead, the user may want to know if there exists any coherent slices that are problematic, as defined by satisfying a rule: has accuracy less than some threshold, and number of examples above some threshold.  Therefore, we also propose a procedure that recursively clusters influence embeddings until slices satisfying the rule are found, or until the slices are too small.  The approach is analogous to building a tree to identify slices satisfying the rule, where the splits are determined by K-Means clustering of influence embeddings.  In addition to letting the user specify more intuitive hyperparameters, this procedure also has the advantage that if a large slice with sufficiently low accuracy is found, it will not be clustered further.  Algorithm \ref{alg:rule} in the Appendix outlines this \texttt{InfEmbed-Rule} method.  Its inputs are the same as \texttt{InfEmbed}, except instead of $K$, the number of slices, one specifies accuracy threshold $A$, size threshold $S$, and branching factor $B$, which specifies how many clusters the K-means call in each step of the recursion should return.  Its output is a set of slices, each having accuracy less than $A$ and size greater than $S$.  %In practice, the recursion proceeds to a maximum depth.

\subsection{Properties of Discovered Slices}\label{sec:properties}
Existing SDMs \cite{eyuboglu2022domino, hua2022discover} explicitly encourage slices to have a \emph{label homogeneity} property---that a given slice is homogeneous in terms of both the true and predicted label, relying on ``error-aware'' mixture models of examples' features, predicted label, and true label.  This requires tuning a hyperparameter trading off homogeneity in labels versus that in features.  

In contrast, our procedure is able to achieve label homogeneity by simply applying K-Means to influence embeddings without any hyperparameter.  This is because K-Means encourages influence embeddings within the same slice to have low Euclidean distance, which is in turn their negative dot-product plus a constant.  Therefore, we consider what factors results in two examples $z=(x,y)$, $z'=(x',y')$ having influence embeddings with high dot-product.  For simplicity, we consider when the dot-product of their \emph{gradients} would be high; influence embeddings are linearly transformed gradients (see Equation \ref{eq:emb}), and high dot-product before transformation implies high dot-product after transformation.  For further simplicity, we consider the case when the model $f$ is a linear model, so that $f(x;\theta)=\theta^{\intercal}x$, where $\theta=[B_1,\mydots,B_C]$, linear coefficient vectors for each class.  

Given that $L$ is cross-entropy loss, we define $p\coloneqq[p_1,\mydots,p_C]=\operatorname{softmax}(f(x))$, the predicted probabilities for each class for example $z$, and define $p'$ analogously for example $z'$.  A simple calculation shows $\nabla_{\theta}L(z;\theta) = [(1[y_1\shorteq 1]\shortsub p_1)x,\mydots,(1[y_C\shorteq 1]\shortsub p_C)x]$, where $y_c$ indicates whether the label is class $c$.  Thus,
\begin{align}
\nabla_{\theta}L(z;\theta)^{\intercal}\nabla_{\theta}L(z';\theta) = (y - p)^{\intercal}(y'-p') x^{\intercal}x'.\label{eq:truth}
\end{align}
Note that $y-p$ is the \emph{margin} for example $z$---the vector containing the difference between true label and predicted probability for each class (and similarly for $y'-p'$).  Thus, clustering influence embeddings leads to label homogeneity due to the use of gradients. The gradients of two examples are similar by dot-product when their margins are similar by dot-product, which occurs if their true labels and predicted probabilities are similar.

Equation \ref{eq:truth} also shows that in the simple case of a linear model, our method considers the dot-product between the last-layer activations, i.e. input features for this case.  However, in the more general case, unlike past slice discovery methods relying on last-layer activations, our method considers information in other layers of the model simply by virtue of considering gradients in them.


\subsection{Root-Cause Analysis via Slice Opponents}
\label{sec:method:proponents}
Given an under-performing slice, we are interested in identifying the root-cause of the erroneous predictions in that slice. As the root-cause, we compute the strongest \textit{opponents} of the slice.  These opponents are the training examples whose influence on the \emph{slice}, i.e. influence on the \emph{total} loss over all examples in the slice is the most negative, i.e., most harmful.  Due to the properties of influence embeddings, the influence of a training example on a slice is simply the dot-product between the influence embedding of the training example, and the \emph{sum} of the influence embeddings in that slice. Inspecting slice opponents can provide insight into the key features responsible for low performance in a slice.

==> sections/old/introduction.tex <==
%\vspace*{-18pt}
\section{Introduction}
\juliusad{This is the workshop introduction. It is nice, but I think we should do the old icml introduction since that has more hand holding.}
Error discovery is a longstanding challenge in machine learning~\citep{pope1976statistics, amershi2015modeltracker, sculley2015hidden, chung2019automated, chakarov2016debugging, cadamuro2016debugging,  kearns2018preventing, kim2019multiaccuracy, zinkevichrules2020}. Recently, \citet{eyuboglu2022domino} formalized a type of error analysis termed the \emph{slice discovery problem}. In the \emph{slice discovery problem}, given a pre-trained multi-class classification model and test data, the goal is to partition the \emph{test} data into a set of \emph{slices}---groups of test examples---on the basis of both their features and labels.  An effective slice discovery method (SDM) should satisfy two desiderata:
%\vspace{-2mm}
\begin{enumerate}
\itemsep0em
\item \emph{Error surfacing}: Identify \emph{under-performing slices}, i.e. slices with low accuracy, if they exist.
\item \emph{Coherence}: Return slices that are \emph{coherent} in the following sense: Erroneous predictions in a given slice should have the same \emph{root cause}, i.e. be ``wrong for the same reason''.
\end{enumerate} 

In developing a SDM, there are two key challenges: 1) \emph{Formalizing the coherence property}: defining the \emph{root cause} of an error, identifying whether two errors have similar root causes, and ultimately, defining whether a slice is \emph{coherent}; and 2) \emph{Identifying the representation to use}, i.e., given two samples, for which a model gives the wrong prediction, the basis of comparison to assess the similarity of the cause of the error for both samples.

 In this paper, we tackle those challenges and contribute the following:
 %\vspace{-10pt}
 \begin{enumerate}
\itemsep0em
     \item \textbf{A new slice discovery method}: We propose $\texttt{InfEmbed}$, a SDM to identify under-performing slices that applies K-Means to a new representation: \emph{influence embeddings}.
     
     \item \textbf{Coherence \& Theoretical Justification.} We formalize the \textit{coherence property}, which requires that erroneous predictions within a slice should be ``wrong for the same reason''.  We then define influence embeddings, and theoretically show that a procedure which clusters them achieves coherence in a sense made precise by leveraging influence functions: it returns slices whose examples are \emph{influenced similarly by the training data.}

     \item \textbf{Empirical Performance.} We show that $\texttt{InfEmbed}$ outperforms previous state-of-the-art SDMs on the DCBench benchmark ~\citep{eyuboglu2022dcbench}. $\texttt{InfEmbed}$ is scalable, able to recover known errors in variety of settings, and identifies coherent slices on realistic models.
 \end{enumerate}

==> sections/pseudocode.tex <==
\algnewcommand{\LeftComment}[1]{\Statex \(\triangleright\) #1}
\begin{algorithm}
\label{alg:arnoldi_factor}
\caption{Finding low-rank factors of Hessian}
\begin{algorithmic}
\Procedure{FactorHessian}{$\tr{\mybold{Z}}$, $\Theta$, $P$, $D$}
\State\textbf{Inputs:} training data $\tr{\mybold{Z}}$, configuration $\Theta$, Arnoldi dimension $P$, rank $D$
\State $H_\theta \gets \sum_{i=1}^{N'} \nabla_{\theta}^2 L(\idx{\tr{z}}{i};\theta)$ \Comment{implicitly define HVP}
\State Run Arnoldi iteration on $H_\theta$ for $P$ iterations to get $Q\in \mathbb{R}^{|\theta| \times P}, R\in \mathbb{R}^{P\times P}$
\State $V, \lambda \gets$ top-$D$ eigenvectors / values of $R$ via SVD
\State $M \gets QV$
\State \textbf{Return:} $M, \lambda$
\EndProcedure
\end{algorithmic}
\end{algorithm}
\juliusad{Let's move the algo to apdx if poss.}
